Can I use this publicly available dataset to build commercial AI software? -- A Case Study on Publicly Available Image Datasets

Publicly available datasets are one of the key drivers for commercial AI software. The use of publicly available datasets is governed by dataset licenses. These dataset licenses outline the rights one is entitled to on a given dataset and the obligations that one must fulfil to enjoy such rights without any license compliance violations. Unlike standardized Open Source Software (OSS) licenses, existing dataset licenses are defined in an ad-hoc manner and do not clearly outline the rights and obligations associated with their usage. Further, a public dataset may be hosted in multiple locations and created from multiple data sources each of which may have different licenses. Hence, existing approaches on checking OSS license compliance cannot be used. In this paper, we propose a new approach to assessing the potential license compliance violations if a given publicly available dataset were to be used for building commercial AI software. We conduct a case study with our approach on 6 commonly used publicly available image datasets. Our results show that there exists potential risks of license violations associated with all of the studied datasets if they were used for commercial purposes.

==> Sections/04-AILifecycle.tex <==
\section{The impact of copyright and contract issues on the AI Software Development Lifecycle}~\label{sec:ailifecycle}
%\begin{figure*}[htp]
%    \centering
%    \includegraphics[width=\textwidth]{Figures/ailifecycle.pdf}
%    \caption{The potential ways in which the contract and copyright issues can impact the different stages of AI software development lifecycel. The AI software development lifecycle is adopted from Amershi et al.~\cite{amershi2019software}\gopi{If we run out of space, I think this figure can be removed}}
%\end{figure*}

In this section, we outline how the different steps of AI software development life cycle proposed by Amershi et al.~\cite{amershi2019software} could be impacted by a copyright and the contractual issues that the use a publicly available dataset may engender. We do so by explaining how the presence of copyright issues or contractual issues may impact a given AI software development stage. 

To better explain the issues that may occur, we use an example of a case where CIFAR-10 dataset is used to develop an AI software in the commerical context. CIFAR-10 is one of the most widely used AI datasets[]. Except a request for citation, the creators of CIFAR-10 dataset do not place any explicit restrictions on how the dataset maybe used. CIFAR-10 dataset is collection of 60,000 32*32 color images representing 10 classes (i.e., airplanes, cars, birds, cats, deer, dogs, frogs, horses, ships, and trucks). There are 6000 images per class. The CIFAR-10 dataset is a subset of the 80 Million tiny images dataset, which was in turn extracted by querying Google Images, Flickr, AltaVista, Ask, Cydral and Webshots search engines. 

\smallskip\noindent\textbf{Potential copyright issues in CIFAR-10.} CIFAR-10 dataset may have images that are protected by copyrights. The 80 Million tiny images dataset from which CIFAR-10 was derived downloaded images from the search engines mentioned above without any filters to remove copyrighted images~\cite{torralba200880}. 

\smallskip\noindent\textbf{Potential contractual issues in CIFAR-10.} CIFAR-10 dataset's lack of explicit license places the dataset under copyright law of Canada (since, CIFAR-10 was created in Canada). When there is no explicit license associated with the dataset, the Canadian copyright law (similar to the U.S copyright law) may apply since datasets are considered as compilations and may as such be protected by copyright laws~\cite{scassa2018data}. In such a case, all rights pertaining to the use of dataset lies with the creators of the dataset and actions maybe only allowed at the dataset owner's discretion (except for fair use/fair dealing). 
In addition, CIFAR-10 has images collected from search engines like Google Images which has its own license to content extracted from their search engines, which may also limit what one can do with the CIFAR-10. For instance, Google Images terms of use clearly states that `` You may not modify, rent, lease, loan, sell, distribute or create derivative works based on this Content (either in whole or in part) unless you have been specifically told that you may do so by Google or by the owners of that Content, in a separate agreement". Such a statement further limits actions that we may perform on the images available in the CIFAR-10 dataset. 

\smallskip\noindent\textbf{Model requirements.} During this stage the developers decide which features need to be included and which features can and cannot be implemented for the AI software that is being built. Both copyright and contractual issues might seriously limit what features and models can be built using a given dataset.

\smallskip\noindent\textbf{Running example.} For instance, consider that the AI software that is being built is a AI art generation software which has requires a style transfer feature. The style transfer feature seeks to impose style found in one image onto another image []. In since CIFAR-10 dataset may contain copyrighted images, training a style transfer AI model as a part of our AI software with CIFAR-10 might might be problematic. Similarly, if we want to be able to distribute the dataset as a part of our AI software, we might not be able to do so as the contractual issues may not allow it. 

\smallskip\noindent\textbf{Data collection, cleaning, labeling and feature engineering.} During this stage, the developers collect the required dataset (i.e., oftentimes the publicly available datasets) and then clean the dataset (if required). Then, if the ground truth labels are not already available for the given dataset, the developers label them. Finally, informative features are extracted from the given dataset by selecting or transforming the data points to enhance the performance of the AI models in the AI software. Copyright and contractual issues might impact all of these aforementioned activities as they may explicitly prevent one from modifying, transforming, adding or creating any new content based on the dataset. 

\smallskip\noindent\textbf{Running example.} For our example, as Li et al.~\cite{li2017universal} show we might have to transform our images in the CIFAR-10 dataset using feature transformation like whitening in order to build a successful style transfer AI model. From the copyright issues perspective, simple transformations like whitening may not qualify as derivative work and therefore using the copyrighted images might still constitute as potential infringement. From the contractual issues standpoint, as we explain earlier, the CIFAR-10 images that were collected from Google Images do not allow for any modifications or creation of derivative work per its contract. Therefore, even if whitening constitute as derivative work, transforming the images of CIFAR-10 obtained via Google Images would still constitute as contract violation. 


\smallskip\noindent\textbf{Model training, evaluation and deployment.} During this stage the developers train and evaluate the AI model that is used to build the AI software. Once evaluated, these models along with the AI software are deployed in the real world. Contractual and copyright constraints may govern if an AI model can be trained on given dataset can be deployed for the intended context. 

\smallskip\noindent\textbf{Running example.} For our example, we want to use the AI software trained on CIFAR-10 in a commercial context. However, presence of copyrighted images in CIFAR-10 and the limitations enforced by contract (as we explained previously) limits our ability to deploy the software commercially as we do not have explicit permission from the copyright owners or from the search engines that provided CIFAR-10 with the images.

\smallskip\noindent\textbf{Model monitoring.} During this stage the deployed AI software is monitored for any errors. This stage, since it does not use the dataset actively is not impacted by copyright or contractual issues that may arise from using the publicly available datasets. 

In summary, most stages of the AI software development might be impacted by the copyright and contractual issues that may arise from using the publicly available datasets 


==> Sections/2.5-Motivation.tex <==
\section{Motivation}~\label{sec:motivation}
\jack{I feel section 2 should just be background and related work, some of the content here should be moved to there} 

\jack{Proposed breakdown for the background and related works section:
(1) AI software development overview (explain the importance of dataset, various types of datasets and their industry, and say briefly among them open datasets is very popular)
(2) Legal Rights and Protection on Data;
(3) Objectives associated with analyzing dataset compliance
(4) Existing dataset licenses (terms of use, copyright notices, and some standard dataset licenses (permissive vs. copyleft licenses). Explain with some examples and their challenges/problems (e.g., hard to locate license, multiple copies, data curation process & nested licenses, ambigious terms in the licenses)
(5) Existing work on 
- license compliance analysis (OSS license violation, explain the differences between OSS and dataset - not standardized licenses, lack of Provence/linage info) 
- extracting and analyzing legal requirements (privacy work)
- the legal compliance of dataset licenses (Montreal data license, and one other work i sent to you before?) 
}

\jack{Have this as a subsection within Background, called as ``Legal Rights and Protection on Data''. 
(1) This part you have to outline the data ownerships and rights. In particular, data by itself cannot be share unless explicitly stated. 
(2) Furthermore, whether we can use a particular dataset is generally governed by two sets of law: copyright and contract law.\erika{replace "contract" with "license" here?} What are they, and examples. 
(3) Discuss the breakdown of the licenses for a dataset: about individual work (images), collection work (raw image datasets), and derived work (e.g., labels, etc.) 
(4) What does License enable others to do (e.g., rights, obligations, limitations) 
(5) some law suits or issues with copyright (e.g., Google case)/license violations (e.g., megaface example, etc.)}
Ensuring regulatory compliance in AI software systems is pivotal across the globe. As a part of ensuring regulatory compliance, it is important for constructed AI systems not to violate any license~\cite{ingolfo2013arguing,breaux2008analyzing,kiyavitskaya2008automating,zeni2015gaiust}. When a AI software uses a publicly available dataset, it is implicit that the owners of the AI software enter into an agreement with the copyright holders of the dataset. Such an agreement entails that the AI software system use the datatset only per the rights provided by the license and follow the obligations outlined in them, which in turn makes the obligations a system requirement~\cite{ingolfo2013arguing}. If the AI software system fails to do so, it will be in breach of license--- which becomes an issue of regulatory compliance. As several prior studies note, organizations that are found non-compliant of laws and regulations face serious consequences. Therefore, compliance is both a functional and non-functional requirement of a AI software system. However, as Benjamin~et~al.~\cite{benjamin2019towards} outlines licenses associated with the publicly available datasets do not clearly outline the rights and obligations associated with them. Such a problem makes it hard for the AI engineers to encode these obligations as requirements.

\jack{Have this subsection as ``Objectives and Challenges associated with analyzing the compliance of dataset licenses''
(1) the goal of analyzing licenses from various dataset is to verify if the dataset is suitable for developing commerical AI software systems. 
(2) the extracted rights, obligations, and limitations will be encoded as part of the system requirements. However, conducting compiliance is hard, hence we have the concept of due diligence 
(3) the goals of this work is to propose process to conduct the work, and standardize documentation approaches on our analysis results, and subsequently system requirements; so that we can demonstrate and establish due dilligence} As Breaux~et~al.~\cite{breaux2008analyzing} point out, when requirements, in particular legally enforceable requirements are ambiguous it is important for the AI engineers to do their\textit{due diligence} or take \textit{due care} to make sure their systems are compliant. In other words, AI engineers should make reasonable efforts to make sure that the AI software system is not found in breach of license. To make such a claim AI engineers should employ traceablity from the rights and obligations in the license to system requirements~\cite{breaux2008analyzing,kiyavitskaya2008automating}. In addition, it is imperative for the AI engineers to justify that their interpretation of the rights and obligations is consistent with how they implemented those requirements in the constructed AI software system~\cite{breaux2008analyzing}. Therefore, to justify that the AI engineers do their due diligence to ensure that a constructed AI system does not violate a datasets' license. A rigours method, like the one we propose in our paper that ascertains the rights and obligations associated with a publicly available dataset is vital. 
